SplatAD: Real-Time Lidar and Camera Rendering with 3D Gaussian Splatting for Autonomous Driving

Ensuring the safety of autonomous robots, such as self-driving vehicles, requires extensive testing across diverse driving scenarios. Simulation is a key ingredient for conducting such testing in a cost-effective and scalable way. Neural rendering methods have gained popularity, as they can build simulation environments from collected logs in a data-driven manner. However, existing neural radiance field (NeRF) methods for sensor-realistic rendering of camera and lidar data suffer from low rendering speeds, limiting their applicability for large-scale testing. While 3D Gaussian Splatting (3DGS) enables real-time rendering, current methods are limited to camera data and are unable to render lidar data essential for autonomous driving. To address these limitations, we propose SplatAD, the first 3DGS-based method for realistic, real-time rendering of dynamic scenes for both camera and lidar data. SplatAD accurately models key sensor-specific phenomena such as rolling shutter effects, lidar intensity, and lidar ray dropouts, using purpose-built algorithms to optimize rendering efficiency. Evaluation across three autonomous driving datasets demonstrates that SplatAD achieves state-of-the-art rendering quality with up to +2 PSNR for NVS and +3 PSNR for reconstruction while increasing rendering speed over NeRF-based methods by an order of magnitude. See https://research.zenseact.com/publications/splatad/ for our project page.

==> assets/ablations_pandaset.tex <==
\begin{table}[t]
    \centering
    \caption{PandaSet ablations.}
    \addtolength{\tabcolsep}{-2pt}
    \vspace{-2mm}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{clccccccc}
    \toprule
        &                   & PSNR $\uparrow$  & SSIM $\uparrow$ & LPIPS $\downarrow$ & Depth $\downarrow$ & CD $\downarrow$ & Camera MP/s $\uparrow$ & Lidar MR/s $\uparrow$  \\
       & Full model          & 26.77 & 0.815 & 0.193 & 0.02 & 2.0 & 121.0 & 19.6  \\ \midrule
       b) & Camera RS           & 26.47 & 0.807 & 0.201 & 0.03 & 2.0 & 122.2 & 19.3   \\
       c) & CNN decoder         & 26.32 & 0.804 & 0.212 & 0.03 & 2.1 & 123.1 & 19.7   \\
       e) & EWA                 & 26.74 & 0.810 & 0.223 & 0.06 & 1.3 & 121.4 & 19.6   \\
       f) & Appearance emb.     & 26.36 & 0.802 & 0.206 & 0.03 & 2.3 & 123.2 & 19.8   \\
       g) & Velocity refinement & 26.74 & 0.814 & 0.195 & 0.03 & 2.0 & 120.2 & 19.3   \\
       i) & Lidar RS            & 26.58 & 0.811 & 0.196 & 0.03 & 2.2 & 120.7 & 20.7   \\
       k) & MCMC                & 26.73 & 0.815 & 0.200 & 0.02 & 1.3 & 130.8 & 24.6   \\

    \bottomrule
    \end{tabular}
    }
    \addtolength{\tabcolsep}{2pt}
    \label{tab:pandaset_ablations}
    \vspace{-2mm}
\end{table}

==> assets/nvs_table.tex <==
\begin{table*}[t]
    \centering
    \caption{NVS results for image and lidar point clouds, over three datasets. $^\mathsection$without missing points.  \colorbox{tabfirst}{First}, \colorbox{tabsecond}{second}, \colorbox{tabthird}{third}.}
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{ll ccc cccc ccc}
    
    \multicolumn{2}{c}{} & \multicolumn{3}{c}{Image} & \multicolumn{4}{c}{Lidar} & \multicolumn{3}{c}{Efficiency} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-9} \cmidrule(lr){10-12}
    &     &  PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ 
    & Depth $\downarrow$ & Intensity $\downarrow$ & Drop acc. $\uparrow$ & CD $\downarrow$ 
    & Camera MP/s $\uparrow$ & Lidar MR/s $\uparrow$ & Train time (H) $\downarrow$ \\ \midrule
    \multirow{6}{*}{\rotatebox[origin=c]{90}{\shortstack[c]{\small PandaSet}}}
& UniSim              & 23.12                     & 0.682                      & 0.360                      & \cellcolor{tabsecond}0.08 & \cellcolor{tabthird}0.086  &    -                      & \cellcolor{tabthird}10.3$^\mathsection$&                     11.5   & \cellcolor{tabsecond}0.9  & \cellcolor{tabfirst}0.9\\
& NeuRAD              & \cellcolor{tabsecond}25.80& \cellcolor{tabsecond}0.753 & \cellcolor{tabsecond}0.250 & \cellcolor{tabfirst}0.01  & \cellcolor{tabsecond}0.063 & \cellcolor{tabsecond}96.2 & \cellcolor{tabsecond}1.9                &   9.7                      & \cellcolor{tabsecond}1.1  & \cellcolor{tabthird}1.3\\
& PVG                 & 24.01                     & 0.712                      & 0.452                      & 38.74                     &   -                        &    -                      & 125.2$^\mathsection$                    & \cellcolor{tabsecond}28.2  & \cellcolor{tabthird}0.2   & 1.6\\ 
& Street-GS           & \cellcolor{tabthird}24.73 & 0.745\cellcolor{tabthird}  & \cellcolor{tabthird}0.314  & 6.18                      &   -                        &    -                      & 37.3$^\mathsection$                     & \cellcolor{tabthird}22.8   & \cellcolor{tabthird}0.2   & 2.3\\
& OmniRE              & \cellcolor{tabthird}24.71 & 0.745\cellcolor{tabthird}  & \cellcolor{tabthird}0.315  & \cellcolor{tabthird}2.88  &   -                        &    -                      & 29.8$^\mathsection$                     &    16.5                    & \cellcolor{tabthird}0.2   & 2.6\\
& {\modelname} (ours) & \cellcolor{tabfirst}26.76 & \cellcolor{tabfirst}0.815  & \cellcolor{tabfirst}0.193  & \cellcolor{tabfirst}0.01  & \cellcolor{tabfirst}0.059  & \cellcolor{tabfirst}96.7  & \cellcolor{tabfirst}1.6                 & \cellcolor{tabfirst}121.5  & \cellcolor{tabfirst}19.5  & \cellcolor{tabsecond}1.0\\
    \midrule
    
    \multirow{6}{*}{\rotatebox[origin=c]{90}{\shortstack[c]{\small Argoverse2}}}
& UniSim              &                    22.35   &                    0.655   &                    0.458   & \cellcolor{tabsecond}0.18 & \cellcolor{tabthird}0.081  &                    -	  & \cellcolor{tabthird}29.2$^\mathsection$ &                      10.0 & \cellcolor{tabsecond}0.7    & \cellcolor{tabfirst}1.1\\ 
& NeuRAD              & \cellcolor{tabsecond}26.18 & \cellcolor{tabthird}0.721  & \cellcolor{tabsecond}0.310 & \cellcolor{tabfirst}0.02  & \cellcolor{tabsecond}0.058 & \cellcolor{tabsecond}92.2 & \cellcolor{tabfirst}2.6                 &                      9.7  & \cellcolor{tabsecond}0.9    & \cellcolor{tabthird}1.3\\ 
& PVG                 &                      24.47 &                      0.712 &                    	0.502 &                 -  		   &      -             	    &         -               &       -                                 & \cellcolor{tabsecond}48.0 &    -                        & 2.5\\ 
& Street-GS           &                      25.52 & \cellcolor{tabsecond}0.754 & \cellcolor{tabthird}0.374  &                 -  		   &      -                     &      -                  &    -                                    &  \cellcolor{tabthird}38.7 &    -                        & 2.6\\ 
& OmniRE              & \cellcolor{tabthird}25.61  & \cellcolor{tabsecond}0.753 & \cellcolor{tabthird}0.375  &                 -  		   &      -                     &      -                  &    -                                    &                      23.9 &         -                   & 3.0\\ 
& {\modelname} (ours) & \cellcolor{tabfirst}28.42  & \cellcolor{tabfirst}0.826  & \cellcolor{tabfirst}0.270  & \cellcolor{tabfirst}0.02  & \cellcolor{tabfirst}0.052  & \cellcolor{tabfirst}92.6  & \cellcolor{tabsecond}2.8                & \cellcolor{tabfirst}134.5 & \cellcolor{tabfirst}9.5     & \cellcolor{tabsecond}1.2\\ 
    \midrule

    \multirow{6}{*}{\rotatebox[origin=c]{90}{\shortstack[c]{\small nuScenes}}}
& UniSim              &                     22.66  &                     0.743  &                     0.414  & \cellcolor{tabthird}0.06   & \cellcolor{tabthird}0.063  &                       -   &                     52.2$^\mathsection$ &                      13.3	& \cellcolor{tabsecond}1.0  & \cellcolor{tabfirst}0.7\\ 
& NeuRAD              & \cellcolor{tabsecond}26.17 & \cellcolor{tabsecond}0.790 & \cellcolor{tabsecond}0.312 & \cellcolor{tabfirst}0.01   & \cellcolor{tabsecond}0.042 & \cellcolor{tabsecond}93.1 & \cellcolor{tabthird}6.3	             &                      11.8	& \cellcolor{tabsecond}1.1  & \cellcolor{tabsecond}1.1\\ 
& PVG                 &                     24.94  & \cellcolor{tabthird}0.768  &                     0.497  &                     10.34  &                       -    &                       -   &                     77.9$^\mathsection$ & \cellcolor{tabthird}18.8     & \cellcolor{tabthird}0.02   & 1.4\\ 
& Street-GS           & \cellcolor{tabthird}25.54  & \cellcolor{tabsecond}0.799 & \cellcolor{tabthird}0.375  &                     1.56   &                       -    &                       -   & \cellcolor{tabsecond}4.5$^\mathsection$ & \cellcolor{tabsecond}21.5    & \cellcolor{tabthird}0.04   & 1.6\\ 
& OmniRE              &                     25.50  & \cellcolor{tabsecond}0.798 &                     0.386  &                     1.71   &                       -    &                       -   & \cellcolor{tabsecond}4.6$^\mathsection$ &                       16.3  	& \cellcolor{tabthird}0.03   & 1.9\\ 
& {\modelname} (ours) & \cellcolor{tabfirst}27.54  & \cellcolor{tabfirst}0.849  &  \cellcolor{tabfirst}0.302 & \cellcolor{tabsecond}0.02  & \cellcolor{tabfirst}0.036  & \cellcolor{tabfirst}93.8  & \cellcolor{tabfirst}1.7	             & \cellcolor{tabfirst}106.1    & \cellcolor{tabfirst}5.7   & \cellcolor{tabthird}1.2\\ 

    \bottomrule
    \end{tabular}
    }
    \label{tab:results_table_nvs}
\end{table*}


